Local Adaptation Improves Accuracy of Deep Learning Model for Automated X-Ray Thoracic Disease Detection : A Thai Study

Despite much promising research in the area of artificial intelligence for medical image diagnosis, there has been no large-scale validation study done in Thailand to confirm the accuracy and utility of such algorithms when applied to local datasets. Here we present a wide-reaching development and testing of a deep learning algorithm for automated thoracic disease detection, utilizing 421,859 local chest radiographs. Our study shows that convolutional neural networks can achieve remarkable performance in detecting 13 common abnormality conditions on chest X-ray, and the incorporation of local images into the training set is key to the model's success. This paper presents a state-of-the-art model for CXR abnormality detection, reaching an average AUROC of 0.91. This model, if integrated to the workflow, can result in up to 55.6% work reduction for medical practitioners in the CXR analysis process. Our work emphasizes the importance of investing in local research of medical diagnosis algorithms to ensure safe and efficient usage within the intended region.

==> 2_litreview_old.tex <==
\section{Background}

\subsection{Chest Radiography}
Chest X-rays (CXR) are projection radiographs of the chest used to diagnose conditions affecting the chest, its contents, and nearby structures. Chest X-ray films are usually saved in Digital Imaging and Communications in Medicine (DICOM) format, which allows high-resolution images to be saved along with metadata such as patient name, gender and age. Radiologists diagnose the film and write up reports to describe visible conditions and store them along with chest X-ray films in the Picture Archiving and Communication System (PACS).

\subsection{Chest X-ray Datasets}
Due to the availability of these picture archiving systems in many hospitals, there have been efforts to create datasets suitable for machine learning study by querying their images, associated structured data and unstructured diagnostic reports. Radiologist reports are written in natural language, hence raw text files must be processed by Natural Language Processing (NLP) algorithms, to transform natural text to ground-truth labels that can be used in supervised machine learning. 

Wang et al. \cite{wang2017nihdataset} initially released the ChestX-ray8 dataset with $108,948$ frontal view X-ray images from $32,717$ unique patients. The dataset divides chest conditions into $8$ classes by text mining the labels from radiologist reports. Negations were done by locating the negation keywords and applying rules to create negation labels. They later re-label the observations into $14$ classes and call the new dataset ChestX-ray14.

Irvin et al. \cite{irvin2019chexpert} proposed a public dataset called CheXpert that contains $224,316$ multi-view chest images from $65,240$ unique patients. They used an automatic labeler that reads doctor reports and categorizes them into $14$ chest observations. The labels provided for each observation are divided into mention, negation and uncertain. They also used an improved version of the labeler over that used by Wang et al. \cite{wang2017nihdataset}. In addition, their labeler used NLP-based tools and was set up in three distinct stages: mention extraction stage which extracts mentions from a list of observations, mention classification stage which classifies extracted mentions into positive, negative and uncertain, and mention aggregation phase, which aggregates classifications into their final $14$ labels. They also improve the negation method by dividing negation phase into pre-negation and post-negation, and including more rules in the negation phase.

Johnson et al. \cite{johnson2019mimic} introduced the MIMIC-CXR dataset of $371,920$ multi-view chest images from $224,548$ unique patients. They also provide doctor reports in addition to the images.

Lastly, Bustos et al. \cite{bustos2019padchest} presented the Padchest dataset with $160,868$ images with their associated reports. $27,593$ of the reports were manually labeled and used to train the labeler to generate labels for the rest of the dataset.

\subsection{Chest X-ray Abnormality Detection with Deep Learning}

In early years, various approaches using image processing techniques have been proposed to detect disease-specific features and identify abnormalities in chest X-ray images.
Dallal et al. \cite{dallal2017imgproc} proposed an approach to assess cardiomegaly condition in patients by measuring the cardiothoracic-ratio (CTR) value. Their approach searches a reference image repository for the nearest neighbor of the patient's sample X-ray image, and a SIFT flow algorithm was used to align and transform the lung boundary from the nearest neighbor image to the sample.
Udeshani et al. \cite{udeshani2011statistical} proposed an approach to detect lung cancer from chest X-ray images. After removing noise from the image, they segment regions suspected to have lung nodules by finding connected components from the image and calculate roundness index for each connected component. A neural network with one hidden layer is then applied on first-order features based on gray levels and second-order features generated from gray level co-occurrence matrix (GLCM) to verify if that region contains a nodule.
Various approaches using image processing techniques were also proposed for screening Tuberculosis from chest X-ray films and were nicely presented in a detailed survey by Dallal et al. \cite{jaeger2013automatic}.
While these approaches work well in the applications they are proposed for, they do not extend well to the detection of other diseases or to other datasets.

Since the introduction of Convolutional Neural Networks (CNNs), various neural network models has been proposed to detect objects with great accuracy and generalizability.
He et al. \cite{he2016deep} introduced ResNet which improves conventional CNNs by introducing residual blocks and skip connections that allow later layers to use activations from early layers, reducing the impact of vanishing gradients.
Huang et al. \cite{huang2017densely} proposed DenseNet, which improves over ResNet by introducing dense blocks. A dense block contains a set of layers that utilize the ideas of dense connectivity, which are connections that allow later layers to fully utilize activation from early layers. By utilizing dense blocks, DenseNet achieves improved results over previous approaches on ImageNet \cite{deng2009imagenet} dataset.
Tan et al. \cite{tan2019efficientnet} proposed EfficientNet, which improves upon traditional scaling of Convolutional Neural Networks (CNNs). By balancing network depth, width, and resolution, they achieve state-of-the-art results on ImageNet \cite{deng2009imagenet} dataset compared with other models using the same parameter count. They also used the swish activation function which was claimed to outperform the traditional ReLU function on trained model accuracy.
Additionally, they performed grid search on their scaling parameters and provided models of various sizes pre-trained on ImageNet ranging from EfficientNet-B1, which has the smallest parameter count, to EfficientNet-B7, with the largest parameter count.
%One of the most popular dataset for training CNN for image-based tasks is ImageNet \cite{deng2009imagenet}. ImageNet is a large scale, hierarchical image database that contains 3.2 million images from various categories. ImageNet is used to pre-train models for various image-based applications, which also include medical imaging.

Research has been conducted on medical abnormality screening from chest X-ray images using CNNs. Unlike image processing-based approaches, these research studies aim to detect every disease with one CNN model, making them more flexible to use and adapt to the detection of new diseases.
In addition to developing the ChestX-ray14 dataset, Wang et al. also evaluate various CNN models on the dataset and measured the accuracy \cite{wang2017nihdataset}. They found that the ResNet-50 model yields greatest results on most chest conditions.
Rajpurkar et al. uses the DenseNet-121 model to detect abnormality in chest X-ray images \cite{rajpurkar2017chexnet}. Images are resized to $224$ by $224$ pixels before they are fed into the network. They evaluated their approach on the ChestX-ray14 dataset and report that findings obtained by their approach achieve comparable results to those made by radiologists and also improved the AUC score over previous approaches.
The class activation mappings (CAMs) \cite{zhou2016learning} from their model applied on chest X-ray images also show regions similar to those radiologists use to diagnose chest X-ray images.
Irvin et al. uses DenseNet-121 with CheXpert dataset \cite{irvin2019chexpert}. The model is trained with multi-view chest X-ray images with the resolution of $320$ by $320$ pixels. They compared the performances with three radiologists and reported that their approach achieves comparable performances to radiologists at each of their operating point. They also compared various approaches using uncertainty labels and concluded that treating such labels as positive yielded greatest result on detection of Atelectasis and treating them as a separate class yielded greatest result on detection of Cardiomegaly, and inconclusive on other classes.


%densenet-224 trained on NIH

%densenet-224 trained on chexpert
%densenet-224 trained on NIH

%\subsection{Cardiothoracic Ratio}
%
%%%% [JC] %%%
%% <done> Let's start the background section with CTR and how they are calculated %in general.
%% <done> Please add a citation for your CTR formula.
%% <done> Please add what MRD and MLD stand for.
%%%% [END JC] %%%
%
%%% [KLUI] CTR background
%Chest radiography is the most common tool for detecting cardiomegaly due to the %low cost and high availability of devices to obtain chest X-ray images. From %chest X-ray images, radiologists employ CTR as one of the most important %indicators of cardiomegaly due to the simplicity of the calculation.
%%% [KLUI] MRD/MLD / CTR citation added
%CTR of a chest X-ray image is calculated as cardiac diameter (the diameter of the %heart) divided by the thoracic diameter (the diameter of the chest).
%Specifically, CTR can be calculated from three measurements, $MRD$, the %midline-to-right heart diameter, $MLD$, the midline-to-left heart diameter, and %$ID$, the internal diameter of chest %\cite{mensah2015ctrintro,dimopoulos2013ctrintro}, as
%\begin{equation}
%CTR = (MRD + MLD) / ID,
%\label{eqn:ctr}
%\end{equation}
%where $MRD$ and $MLD$ is measured from the greatest perpendicular diameter from %midline to right and left heart border, respectively. Figure %\ref{fig:ctr_details} visualizes the details of CTR calculation. A CTR value of %$0.5$ is generally considered to indicate the upper limit of normal.
%
%Most Picture Archiving and Communication Systems (PACS) used by radiologists %include tools akin to rulers to ease the process for obtaining these %measurements. However, this manual process is labor and time consuming, and can %be error-prone when radiologists need to assess hundreds of chest X-ray films a %day.
%%% [/KLUI]
%
%\begin{figure}
%    \centering
%    \includegraphics[width=0.4\linewidth]{ctr_calculation/CTR_calculation-details%.png}
%    \caption{Figure depicting MRD, MLD, and ID measurements}
%    \label{fig:ctr_details}
%\end{figure}
%
%%Our approach first determines three lengths, $MRD$, $MLD$ and $ID$, using chest %X-ray image segmentation to obtain heart and lung masks. The extents of those %masks are then used to calculate CTR of image.
%
%\subsection{Automated CTR Calculation}
%
%%%% [JC] %%%
%% <done> Please explain a little bit more about other people's works before us. %How do their CTR calculations done exactly??
%% Please review segmentation separately and discuss accuracy of each methods.
%% <klui done> With the current literature it is impossible for readers to judge %how our work is different from previous works.
%%%% [END JC] %%%
%
%There have been several attempts on automatic measurements of cardiothoracic %ratio. These approaches involve the calculation of lung and heart regions in the %image and use extents of the masks to calculate CTR in a similar practice %radiologists use to assess CTR from chest X-ray films.
%
%%%% [JC] %%%
%% Example of literature review for paper [2]
%For the automated segmentation of lung and heart, traditional image processing %methods can achieve great results. In an early work, a reference image repository %was searched for the nearest neighbor of the patient's sample X-ray image, and a %SIFT flow algorithm was used to align and transform lung boundary from the %nearest neighbor image to the sample \cite{dallal2017imgproc}.
%% Please do the same for all papers.
%%%% [END JC] %%%
%
%%%% [KLUI TO BIG]
%% Please add details of segnet here too
%%% [KLUI]
%
%Ebenezer and Rao \cite{ebenezer2017imgproc} applied a Euler number-based approach %to find the best threshold that separates the two lungs from the background. %After removing background regions from four corners of the image and applying %dilation and erosion for image smoothing, thoracic diameter, $ID$, is then %calculated by scanning for leftmost and rightmost points on the lung mask. $MRD$ %and $MLD$ are then calculated from the widest point between two lung masks.
%
%Candemir et al. \cite{candemir2016svm} registers the input chest image with the %most similar image in the model dataset. The similarity is measured by %calculating Bhattacharyya distance of the X-ray intensity histograms. A %correspondence map is then calculated using a SIFT flow algorithm to compute a %transformation matrix, which is applied to the model mask to transform it into %the input image space. CTR value is then calculated from the boundaries of lung %and heart masks.
%
%Recent works show excellent results by applying a deep learning approach called %U-Net to extract lung and heart boundaries \cite{que2018cardioxnet}. This %approach obtained $93.75\%$ accuracy on cardiomegaly detection task, on the %dataset of $103$ images from NIH Chest X-ray Dataset \cite{wang2017nihdataset}.
%Li et al. \cite{li2019automatic} used U-Net to segment heart and lung masks. They %applied a Conditional Random Field to the masks to smooth region boundaries and %calculate CTR by measuring the cardio and thoracic diameters from the lung and %heart masks. They performed the test on $5,000$ postero-anterior (PA) chest X-ray %images from the Radiology Imaging Center in their hospital and obtained $95.3\%$ %accuracy on cardiomegaly detection.
%%%% [IC] %%%
%% I've added this introduction to image segmentation
%%%% [END IC] %%%
%Given the success of image segmentation on CTR calculation, we further explore %image segmentation approaches using deep learning.
%
%%%%
%%Early works apply image processing techniques to calculate such masks. %\cite{dallal2017imgproc, ebenezer2017imgproc} uses image processing techniques to %extract features from lung and heart segments. \cite{candemir2016svm} utilizes %SVM to extract lung and heart boundaries from chest X-ray films. Recent works %show excellent results by applying a deep learning-based segmentation approach to %calculate lung and heart masks  \cite{que2018cardioxnet,li2019automatic}.
%%%%
%
%\subsection{Image Segmentation with Deep Learning}
%Image segmentation has been one of the most active and sought-after fields of %research due to its various applications such as scene understanding, %content-based image retrieval, or medical imaging. In the early years, computer %vision-based approaches were established for various image segmentation tasks. %Although these techniques are accurate on their target tasks, many of them are %not easy to train and adapt to new tasks. We refer readers to a comprehensive %survey by Zaitoun \cite{zaitoun2015imsegsurvey} for further information on early %approaches to image segmentation.
%
%A major breakthrough in image segmentation was made by the introduction of the %deep learning approach.
%U-Net \cite{olaf2015unet} uses a deep learning model to tackle pixel-wise %segmentation tasks accurately with great speed on various segmentation tasks. %U-Net employs an end-to-end encoder-decoder network that contains the encoder %that performs feature extraction from image input and the decoder that processes %the features into output mask. U-Net also concatenates high-resolution features %from encoder parts to the decoder network to improve model localization.
%Segnet \cite{badrinarayanan2017segnet} is an efficient multi-class segmentation %deep learning architecture for scene understanding. Segnet improves computation %time and memory usage with some trade-offs in segmentation accuracy. Segnet %structure consists of encoder and decoder parts. The encoder includes a sequence %of convolutional layers with batch normalization and relu activation function, %and the decoder part mirrors the structure of the encoder.
%
%Iglovikov \cite{iglovikov2018ternausnet} and Balakrishna %\cite{balakrishna2018automatic} further improve the encoder part with VGG11 and %VGG16 networks, respectively.
%
%%%% [IC] %%%
%% I've moved segnet to be in line with U-Net
%%%% [END IC] %%%
